BPE Gets Picky: Efficient Vocabulary Refinement During Tokenizer Training

Language models can largely benefit from efficient tokenization. However, they still mostly utilize the classical BPE algorithm, a simple and reliable method. This has been shown to cause such issues as under-trained tokens and sub-optimal compression that may affect the downstream performance. We introduce Picky BPE, a modified BPE algorithm that carries out vocabulary refinement during tokenizer training. Our method improves vocabulary efficiency, eliminates under-trained tokens, and does not compromise text compression. Our experiments show that our method does not reduce the downstream performance, and in several cases improves it.

==> tex/translation_compression.tex <==
\begin{table}[th!]
    \centering
    \begin{tabular}{cccc}
    \toprule
        \multicolumn{4}{c}{EN-DE Vocabulary size 8192} \\
        \midrule
        T\hphantom{$^{\ast}$} & drop & EN $(\downarrow)$ & DE $(\downarrow)$ \\
        \midrule
        0.6\hphantom{$^{\ast}$} & 805 & 0.9975 & 0.9988  \\
        0.7\hphantom{$^{\ast}$} & 588 & 0.9946 & 0.9955  \\
        0.8\hphantom{$^{\ast}$} & 358 & 0.9956 & 0.9954 \\
        0.9\hphantom{$^{\ast}$} & 160 & 0.9969 & 0.9970 \\
        1.0$^{\ast}$ & 0 & 1      & 1     \\
        \midrule
        \multicolumn{4}{c}{EN-DE Vocabulary size 32768} \\
        \midrule
        T\hphantom{$^{\ast}$} & drop & EN $(\downarrow)$ & DE $(\downarrow)$  \\
        \midrule
        0.6\hphantom{$^{\ast}$} & 2563 & 1.0051 & 1.0005 \\
        0.7\hphantom{$^{\ast}$} & 1970 & 1.0002 & 0.9986 \\
        0.8\hphantom{$^{\ast}$} & 1280 & 0.9984 & 0.9985 \\
        0.9\hphantom{$^{\ast}$} & 677 & 0.9979 & 0.9985 \\
        1.0$^{\ast}$ & 0 & 1      & 1       \\
        \midrule
        \multicolumn{4}{c}{UK-ET Vocabulary size 8192} \\
        \midrule
        T\hphantom{$^{\ast}$} & drop & UK $(\downarrow)$ & ET $(\downarrow)$ \\
        \midrule
        0.6\hphantom{$^{\ast}$} & 605 & 0.9995 & 0.9959  \\
        0.7\hphantom{$^{\ast}$} & 446 & 0.9974 & 0.9948  \\
        0.8\hphantom{$^{\ast}$} & 255 & 0.9954 & 0.9960  \\
        0.9\hphantom{$^{\ast}$} & 107 & 0.9976 & 0.9978  \\
        1.0$^{\ast}$ & 0 & 1      & 1       \\
    \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:mt-compression}
\end{table}
